Exploring Effects of Hyperdimensional Vectors for Tsetlin Machines

Tsetlin machines (TMs) have been successful in several application domains, operating with high efficiency on Boolean representations of the input data. However, Booleanizing complex data structures such as sequences, graphs, images, signal spectra, chemical compounds, and natural language is not trivial. In this paper, we propose a hypervector (HV) based method for expressing arbitrarily large sets of concepts associated with any input data. Using a hyperdimensional space to build vectors drastically expands the capacity and flexibility of the TM. We demonstrate how images, chemical compounds, and natural language text are encoded according to the proposed method, and how the resulting HV-powered TM can achieve significantly higher accuracy and faster learning on well-known benchmarks. Our results open up a new research direction for TMs, namely how to expand and exploit the benefits of operating in hyperspace, including new booleanization strategies, optimization of TM inference and learning, as well as new TM applications.

==> Sections/2_Introduction/Prelim_Tsetlin_Machine.tex <==

\subsection{Tsetlin Machine}


Since its introduction as a pattern recognition paradigm \cite{granmo2018tsetlin}, multiple researchers have proposed extensions to the Tsetlin Machine's initial range of applicability. The convolutional Tsetlin Machine \cite{granmo2019convtsetlin} was proposed as an interpretable alternative to CNNs, using each clause as a convolutional filter that is evaluated against each training image. In contrast to the discreet input/output required by the regular Tsetlin Machine, the Regression Tsetlin Machine\cite{abeyrathna2020nonlinear}. Further, researchers \cite{phoulady2020weighted, abeyrathna2020integer} enabled calculation of individual weights to each clause in order to fine tune the effect of the clauses on the decision making process. Furthermore, once the evaluation of Tsetlin Machine clauses is conducted in parallel, it leads to massive reduction in computation time.\cite{abeyrathna2021massively}. However, their reliance on effective Booleanization strategies presents a challenge. 
%One promising approach is to build a set of concepts, like a set of words in natural language. However, one then needs a single Boolean per concept, e.g., pixel color, phrase, atom, value, or sound. For example, a natural language vocabulary of $10~000$ phrases requires a Boolean vector of $10~000$ values. For complex problems, there can be millions of unique structures, like all possible pixel configurations in an image or all possible sub-structures of chemical compounds. Indeed, certain structures may be of arbitrary size, such as a sentence or a graph, while the input vector of a vanilla TM is fixed.
%More recently, the concept of drop clauses were proposed to enhance the interpretability and the performance of Tsetlin Machines in various classification tasks \cite{sharma2021drop}. Despite all the progress in the various aspects of the Tsetlin Machine that contribute to better performance, both in terms of results as well as resources, the TM has not always performed well in multi-class scenarios. This has been attributed to the fact that during learning, while the TM gives utmost importance to identifying the clauses that support a particular class, the reverse is not always true. i.e. The TM sometimes fails to identify the correct opposing class to learn evidence \textit{against} the class under consideration. This leads to classification mistakes made by the TM specially when the class boundary is not well defined.

%Challenge / what is missing in state of the art
%

% Solution approach

%In this paper, we propose a novel hypervector-based method for addressing the above challenge. A hypervector encodes complex data in a hyperspace of arbitrarily high dimension. This drastically expands    the capacity and flexibility of the TM because in hyperspace, one can use binding and bundling of concepts to easily represent complex data structures, like key-value tuples, sequences, and graphs. Using merely two hyper-Booleans per concept, the TM input space grows quadratically. For instance, a hypervector of size $10~000$ has storage capacity $99~990~000$. When operating in hyperspace, the TM builds logical expressions across the diverse structures, allowing it to reason across an arbitrary number of dimensions.

% Results

%Using the new method, we then demonstrate how to encode images, chemical compounds, and natural language text to achieve significantly higher accuracy and faster learning on well-known benchmarks. For MNIST, we can reduce the number of clauses 10 times, while still outperforming the vanilla TM accuracy-wise, in 10 times fewer epochs. For chemical compounds, we can achieve competitive accuracy in predicting HIV activity from graph sub-structures where resulting hypervector TM models were more robust to the addition of noise, reduced the number of clauses needed as for MNIST and reduced required training times for TM models. ..., and for NLP ... 

 
% Conclusions


%The success of AI models depend is dependant on the internal representation of the data that the model considers. An appropriate representation allows the model to take advantage of the correct juxtaposition of the features available in the data in order to provide the best possible performance that the model is capable of. Moreover, in the case of explainable AI models such as the Tsetlin Machine, this representation also has to be a one-to-one mapping between features that are human understandable and features that are advantageous to the model. In this work, we focus on representation using hypervectors, which represent information in huge dimensional spaces. If the number of
%dimensions is high enough, randomly sampled vectors are expected to be almost
%orthogonal. A hypervector allows us to represent rich and complex information structures, such as lists, graphs, text, image tokens, etc.

%\subsection{Learning in a Multi-class Environment}
%\label{subsec:oldlearning}
%\begin{figure}[ht]
%\centering
%\includegraphics[width=1\linewidth]{figures/tm/Multi-class_Tsetlin_Machine.pdf}
%\caption{Tsetlin Machine in a multiclass scenario}\label{figure:tm_multiclass}
%\end{figure}

%In general the Tsetlin Machine is geared towards binary classification. In many classification tasks however, a multiclass scenario is present, where any observed pattern is to be assigned to one of n classes. Hence the output value $y$ can be one of \{1, . . . , n\}. The Tsetlin Machine tackles multi-class classification problems by representing $y$ in terms of bits and multiple outputs to produce the bit representation of the final class. As shown in Figure. \ref{figure:tm_multiclass}, all the bit level outputs of $y$ are acted upon by a single argmax operator to finally arrive at the prediction. 

%For training, consider we have $y$ = class\_i for a particular observation (X,y). The \ac{TA} representing class\_i are trained as described in \cite{granmo2018tsetlin}. For the second part of the training, a random class, class\_q is chosen as the opposition, such that $q \neq i$. Thus the \ac{TA} for class\_q are trained in accordance to the same scheme applied to TA of $y = 0$ in the binary classification scenario.




==> Sections/4_Empirical_results/emperical_results_artificial.tex <==
\subsection{Artificial}

Show uniqueness of hypervectors using artificial data-----
.....

==> Sections/4_Empirical_results/empirical_results_connect4.tex <==
\subsection{Winner Prediction in Board Games}
%\paragraph{Dataset}
To test the effect of negative sampling on the convergence rate of TM on winner prediction for board game, we experiment on Connect-4 Opening data \cite{blake1998uci}. Connect-4 is a two player strategy board game. The dataset consist of $67,557$  data instances of all legal 8-ply positions for the game of Connect-4. The outcome class is the game theoretical value for the first player, categorized as win, loss and draw. The data is split into train-test set of 77$\%$-33$\%$  Here, we make use of $10,000$ clauses per class with $T=24000$ and $s=100$. Training lasts for 100 epochs.

\setlength\tabcolsep{2.3pt}
\begin{table}[ht]
\caption{\label{tab:connect4_results}Performance comparison of TM with and without Focused Negative Sampling on Connect-4} \centering
\begin{tabular}{c|cc|cc}
\hline
\multirow{2}*{Dataset} & \multicolumn{2}{c}{With FNS} & \multicolumn{2}{c}{without FNS}\\
\cline{2-5} & \bf Num Epochs & \bf Peak Acc. & \bf Num Epochs & \bf Peak Acc.\\\hline
Connect-4 (10\%) & 100 & 83.33  & 100 & 76.71 \\
Connect-4 (100\%) & 100 & 86.22  & 100 & 85.92 \\
\hline
\end{tabular}
\end{table}


\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figures/connect4/connect4_fns_diff.png}
\caption{Performance improvement comparison with between 10\% data and 100\% data for Connect-4 data} \label{fig:FNS_comp_connect4}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figures/connect4/connect4_fns_10501002.png}
\caption{Performance comparison for increasing number of
training samples (in $\%$) with and without FNS for Connect-4 data} \label{fig:FNS_connect4_incr}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[width=\textwidth]{figures/connect4/connect4_fns_on.png}
% \caption{Performance comparison for increasing number of
% training samples (in $\%$) with FNS for Connect-4 data} \label{fig:FNS_connect4_incr}
% \end{figure}
\paragraph{Observations}
As shown in Fig \ref{fig:FNS_comp_connect4} and Table \ref{tab:connect4_results}, FNS achieves an accuracy that is approximately 1\% points better than the non-FNS TM when trained for same number of epochs.

Interestingly, we also observed that training on a very small subset of data i.e., 10\% in our case shows a  high increase in accuracy of 7\% when utilizing FNS, similar to the observation made in subsection \ref{nlp_experiments}. However, increasing the number of training samples to 67k does not yield the same gains of using the FNS as opposed to not using it (Figure \ref{fig:FNS_comp_connect4}). 
Figure \ref{fig:FNS_connect4_incr} compares the accuracy over epochs for TM with vs without FNS for different percentages of training samples.
We hypothesize that this is because the increased available information allows the TM to learn equally effectively in both scenarios. However, this needs to be further verified with more experiments.
%\textcolor{teal}{\textit{Fig10/11 combined?}}

==> figures/tm/TM_Drawing_Formulas.tex <==


\noindent Formulas for the diagram:
\begin{align*}
C^+_1 & = h_1 \land \neg h_2 = 0 \\
C^+_1 & = \neg h_1 \land h_2 = 1 \\
C^+_3 & = h_2 = 1 \\
C^+_3 & = \neg h_1 \land \neg h_2 = 0 \\
\sum C^+ + \sum C^- & = 1 \implies \hat{y} = 1 \\
\sum C^+ + \sum C^- & < \sum C^- \implies \hat{y} = 0 \\
Variables & : h_1, \neg h_1, h_2, \neg h_2 \\
Input & : [h_1, h_2] = [0, 1]
\end{align*}


==> related_work.tex <==
\section{Related Work}

A comparison of vector symbolic architectures \cite{schlegel2022comparison}


MAP-C - Standard/Dense

BSDC-S - Sparse





using TM to 'understand' similarity, and not cosine similarity \cite{steck2024cosine}
